KDFNet: Learning Keypoint Distance Field for 6D Object Pose Estimation

We present KDFNet, a novel method for 6D object pose estimation from RGB images. To handle occlusion, many recent works have proposed to localize 2D keypoints through pixel-wise voting and solve a Perspective-n-Point (PnP) problem for pose estimation, which achieves leading performance. However, such voting process is direction-based and cannot handle long and thin objects where the direction intersections cannot be robustly found. To address this problem, we propose a novel continuous representation called Keypoint Distance Field (KDF) for projected 2D keypoint locations. Formulated as a 2D array, each element of the KDF stores the 2D Euclidean distance between the corresponding image pixel and a specified projected 2D keypoint. We use a fully convolutional neural network to regress the KDF for each keypoint. Using this KDF encoding of projected object keypoint locations, we propose to use a distance-based voting scheme to localize the keypoints by calculating circle intersections in a RANSAC fashion. We validate the design choices of our framework by extensive ablation experiments. Our proposed method achieves state-of-the-art performance on Occlusion LINEMOD dataset with an average ADD(-S) accuracy of 50.3% and TOD dataset mug subset with an average ADD accuracy of 75.72%. Extensive experiments and visualizations demonstrate that the proposed method is able to robustly estimate the 6D pose in challenging scenarios including occlusion.

==> table_ycb.tex <==


\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\vspace{1ex}
\caption{ Results on YCB-Video dataset. Evaluation metric is \textbf{ADD(-S) AUC}. The maximum threshold for AUC is 10cm. }
\begin{tabular}{l|cccc}
\hline
method & PoseCNN \cite{posecnn} & \textbf{KDFNet (ours)} \\
\hline
\texttt{002\_master\_chef\_can}  &  55.2 & \textbf{61.9}
 \\
\texttt{003\_cracker}   & 52.9 &  \textbf{79.5}
 \\
\texttt{004\_sugar\_box}    & 68.3  &  \textbf{81.2}
  \\
\texttt{005\_tomato\_soup\_can}   & 66.1  &  \textbf{72.9}

 \\
\texttt{006\_mustard\_bottle}  & 80.8 &  \textbf{82.6}

 \\
\texttt{007\_tuna\_fish\_can}    & \textbf{70.6} &  48.8

 \\
\texttt{008\_pudding\_box}    & 62.2 &  \textbf{71.2}

 \\
\texttt{009\_gelatin\_box}    & 74.8  &  \textbf{78.8}

 \\
\texttt{010\_potted\_meat\_can}  & \textbf{59.5} &  58.2

 \\
\texttt{011\_banana}  & \textbf{72.1}  & 41.8
  \\
\texttt{019\_pitcher\_base}   & 53.1 &  \textbf{85.3}

 \\
\texttt{021\_bleach\_cleanser}  &  50.2   & \textbf{55.0}

 \\
\texttt{024\_bowl}   &  69.8 & \textbf{73.4}
 \\
\texttt{025\_mug}   &  58.4 &   \textbf{67.9} 
\\
\texttt{035\_power\_drill}    &  55.2  & \textbf{73.5}
 \\
\texttt{036\_wood\_block}   &  61.8 &   \textbf{65.3}
 \\
\texttt{037\_scissors}   &  35.3  &  \textbf{42.1} \\
\texttt{040\_large\_marker}    & \textbf{58.1} & 32.1
 \\
\texttt{051\_large\_clamp}    & 50.1 & \textbf{52.3}
 \\
\texttt{052\_extra\_large\_clamp}   & \textbf{46.5} & 43.7
 \\
\texttt{061\_foam\_brick}  & \textbf{85.9} & 78.9 \\
\hline
average  & 61.0 & \textbf{64.1} \\
\hline
\end{tabular}
\end{table}
